Multi-Armed Bandit Problem with Temporally-Partitioned Rewards: When Partial Feedback Counts

There is a rising interest in industrial online applications where data becomes available sequentially. Inspired by the recommendation of playlists to users where their preferences can be collected during the listening of the entire playlist, we study a novel bandit setting, namely Multi-Armed Bandit with Temporally-Partitioned Rewards (TP-MAB), in which the stochastic reward associated with the pull of an arm is partitioned over a finite number of consecutive rounds following the pull. This setting, unexplored so far to the best of our knowledge, is a natural extension of delayed-feedback bandits to the case in which rewards may be dilated over a finite-time span after the pull instead of being fully disclosed in a single, potentially delayed round. We provide two algorithms to address TP-MAB problems, namely, TP-UCB-FR and TP-UCB-EW, which exploit the partial information disclosed by the reward collected over time. We show that our algorithms provide better asymptotical regret upper bounds than delayed-feedback bandit algorithms when a property characterizing a broad set of reward structures of practical interest, namely alpha-smoothness, holds. We also empirically evaluate their performance across a wide range of settings, both synthetically generated and from a real-world media recommendation problem.

==> contents/07Checklist.tex <==
\section*{Checklist}

\begin{enumerate}
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
		\answerYes{We provide the purpose of the paper and we clarify the novelty in the Original Contributions section and through the discussion of the Related Works. In the first part of the paper, we also summarized the theoretical results.}
		\item Did you describe the limitations of your work?
		\answerYes{The assumptions and scenarios in which our work is valid are listed throughout the paper.}
		\item Did you discuss any potential negative societal impacts of your work?
		\answerNA{This work does not present any foreseeable societal consequence and, to our best knowledge, no one will be put at disadvantage.}
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes{}
	\end{enumerate}
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerYes{We provide each theorem statements with the necessary assumptions for the results to hold.}
		\item Did you include complete proofs of all theoretical results?
		\answerYes{They are provided in Appendix~\ref{a:proof_UB}.}
	\end{enumerate}
	
	\item If you ran experiments...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerYes{We will attach the code corresponding to the experimental section of the paper in the Supplementary Material.}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerNA{Since we are working in an online setting, such a split is not necessary.}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerYes{We performed the experiment multiple times. The plots report error bars representing the confidence interval at $95\%$.}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerYes{They have been reported in Appendix~\ref{a:experiments}.}
	\end{enumerate}
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerYes{We added the reference as asked by the authors at: \url{https://www.aicrowd.com/challenges/spotify-sequential-skip-prediction-challenge}.}
		\item Did you mention the license of the assets?
		\answerYes{The authors allowed its use in academic publication.}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerNo{}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerNA{}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerNA{}
	\end{enumerate}
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
		\answerNA{}
	\end{enumerate}
	
\end{enumerate}
